Warm Jupiters in TESS Full-Frame Images: A Catalog and Observed Eccentricity Distribution for Year 1

Warm Jupiters -- defined here as planets larger than 6 Earth radii with orbital periods of 8--200 days -- are a key missing piece in our understanding of how planetary systems form and evolve. It is currently debated whether Warm Jupiters form in situ, undergo disk or high eccentricity tidal migration, or have a mixture of origin channels. These different classes of origin channels lead to different expectations for Warm Jupiters' properties, which are currently difficult to evaluate due to the small sample size. We take advantage of the \TESS survey and systematically search for Warm Jupiter candidates around main-sequence host stars brighter than the \TESS-band magnitude of 12 in the Full-Frame Images in Year 1 of the \TESS Prime Mission data. We introduce a catalog of 55 Warm Jupiter candidates, including 19 candidates that were not originally released as \TESS Objects of Interest (TOIs) by the \TESS team. We fit their \TESS light curves, characterize their eccentricities and transit-timing variations (TTVs), and prioritize a list for ground-based follow-up and \TESS Extended Mission observations. Using hierarchical Bayesian modeling, we find the preliminary eccentricity distributions of our Warm-Jupiter-candidate catalog using a Beta distribution, a Rayleigh distribution, and a two-component Gaussian distribution as the functional forms of the eccentricity distribution. Additional follow-up observations will be required to clean the sample of false positives for a full statistical study, derive the orbital solutions to break the eccentricity degeneracy, and provide mass measurements.

==> Tables/FP_para.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{llcccccccccl}
\centerwidetable
\tablecaption{False-Positives (FPs) and False-Alarms (FAs) identified by TFOP WG Follow-Up \label{tbl:fp}}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablehead{
\colhead{TIC ID} & \colhead{TOI name} & \colhead{SG1/2 Disposition} & \colhead{R$_\star$} & \colhead{$\rho_\star$} & \colhead{$\rho_{\textrm{circ}}$} & \colhead{$\delta$} & \colhead{$R_{\textrm{p}}$} & \colhead{$b$} & \colhead{$P$} & \colhead{$T_c$} & \colhead{Comments/Reference}\\ 
\colhead{} & \colhead{} & \colhead{} & \colhead{[R$_\sun$]} & \colhead{[$\rho_\sun$]} & \colhead{[$\rho_\sun$]} & \colhead{[ppt]} & \colhead{[$R_\earth$]} & \colhead{} & \colhead{[day]} & \colhead{[BJD-245700]} & \colhead{}
}
\decimalcolnumbers
\startdata
293853437 & TOI-629.01 & BD & 2.177$^{+0.099}_{-0.099}$ & 0.164$^{+0.028}_{-0.028}$ & 0.205$^{+0.031}_{-0.072}$ & 2.119$^{+0.097}_{-0.082}$ & 10.937$^{+0.562}_{-0.549}$ & 0.319$^{+0.264}_{-0.220}$ & 8.717$^{+0.001}_{-0.001}$ & 1463.223$^{+0.002}_{-0.002}$ & - \\
151681127 & TOI-671.01 & SB1 & 1.622$^{+0.049}_{-0.049}$ & 0.340$^{+0.056}_{-0.056}$ & 0.361$^{+0.026}_{-0.022}$ & 14.629$^{+0.204}_{-0.232}$ & 21.392$^{+0.672}_{-0.671}$ & 0.700$^{+0.018}_{-0.023}$ & 10.198$^{+0.001}_{-0.001}$ & 1552.913$^{+0.000}_{-0.000}$ & - \\
55383975 & TOI-694.01 & SB1 & 0.972$^{+0.038}_{-0.038}$ & 1.025$^{+0.132}_{-0.132}$ & 2.892$^{+0.509}_{-0.439}$ & 12.966$^{+0.682}_{-0.620}$ & 12.071$^{+0.560}_{-0.553}$ & 0.570$^{+0.071}_{-0.084}$ & 48.051$^{+0.000}_{-0.000}$ & 1318.722$^{+0.001}_{-0.001}$ & \citetalias{mire20} \\
308050066 & TOI-679.01 & SB1 & 1.813$^{+0.068}_{-0.068}$ & 0.226$^{+0.048}_{-0.048}$ & 0.447$^{+0.047}_{-0.103}$ & 6.773$^{+0.203}_{-0.210}$ & 16.262$^{+0.662}_{-0.658}$ & 0.261$^{+0.220}_{-0.184}$ & 11.176$^{+0.001}_{-0.001}$ & 1552.067$^{+0.001}_{-0.001}$ & - \\
100757807 & TOI-811b & BD & 1.193$^{+0.051}_{-0.051}$ & 0.600$^{+0.106}_{-0.106}$ & 1.990$^{+0.226}_{-0.387}$ & 9.871$^{+0.381}_{-0.351}$ & 12.920$^{+0.608}_{-0.582}$ & 0.267$^{+0.187}_{-0.178}$ & 25.174$^{+0.001}_{-0.001}$ & 1413.080$^{+0.002}_{-0.002}$ & \citetalias{carm20b} \\
231736113 & TOI-1406.01 & BD & 1.235$^{+0.046}_{-0.046}$ & 0.552$^{+0.106}_{-0.106}$ & 0.843$^{+0.204}_{-0.365}$ & 4.295$^{+0.292}_{-0.268}$ & 8.830$^{+0.451}_{-0.431}$ & 0.377$^{+0.271}_{-0.258}$ & 10.574$^{+0.001}_{-0.001}$ & 1404.034$^{+0.003}_{-0.003}$ & \citetalias{carm20a} \\
235067594 & - & NEB & 0.902$^{+0.043}_{-0.043}$ & 1.252$^{+0.154}_{-0.154}$ & 2.129$^{+1.033}_{-1.366}$ & 3.304$^{+0.866}_{-0.413}$ & 5.680$^{+0.705}_{-0.477}$ & 0.485$^{+0.311}_{-0.329}$ & 8.296$^{+0.001}_{-0.001}$ & 1430.649$^{+0.004}_{-0.004}$ & CTOI; \citetalias{mont20}; actual star TIC-235067595 \\
92833442 & - & NEB & 0.853$^{+0.027}_{-0.027}$ & 1.327$^{+0.184}_{-0.184}$ & 2.454$^{+0.797}_{-1.002}$ & 12.813$^{+1.308}_{-1.014}$ & 10.531$^{+0.607}_{-0.544}$ & 0.444$^{+0.229}_{-0.286}$ & 16.205$^{+0.001}_{-0.001}$ & 1506.681$^{+0.001}_{-0.001}$ & actual star TIC-92833424 \\
140344868 & - & NEB & 0.998$^{+0.049}_{-0.049}$ & 0.906$^{+0.163}_{-0.163}$ & 1.253$^{+0.308}_{-0.428}$ & 17.689$^{+1.494}_{-1.217}$ & 14.488$^{+0.918}_{-0.873}$ & 0.382$^{+0.225}_{-0.249}$ & 8.101$^{+0.001}_{-0.001}$ & 1463.662$^{+0.002}_{-0.002}$ & actual star TIC-140344846 \\
425170378 & - & FA & - & - & - & - & - & - & - & - & - \\
\enddata
\tablecomments{BD: Brown Dwarf; SB1: Spectroscopy Binary 1 (single-lined spectra showing RV variation too large to be caused by a planet); NEB: Nearby Eclipsing Binary; FA: False Alarm}
\tablerefs{Reference abbreviations used in this table are listed. Mi20: \cite{mire20}; Ca20a: \cite{carm20a}; Ca20b: \cite{carm20b}; Mo20: \cite{mont20}}
\end{deluxetable*}
\end{longrotatetable}

==> Tables/PC.tex <==
\begin{longrotatetable}
\begin{deluxetable*}{lccccccccccccl}
\centerwidetable
\tablecaption{Warm Jupiter Candidates Discovered in Year 1 \TESS Full-Frame Images. A brief description of the columns: (1) \TESS Input Catalog ID, TIC ID (2) stellar radius in solar radius, $R_\star$ (3) stellar density in the mean solar density, $\rho_\star$ (4) stellar density inferred from light curves assuming a circular-orbit planet in the mean solar density, $\rho_{\textrm{circ}}$ (5) transit depth in parts-per-thousand (ppt), $\delta$ (6) planet radius in Earth radii, $R_{\textrm{p}}$ (7) impact parameter, $b$ (8) orbital period in days, $P$ (9) conjunction time, $T_c$ (10) the mode and 68\% highest posterior density (HPD) interval of the eccentricity, $e$; (11) the 68\% HPD intervals of the argument of periapse in degrees, $\omega$ (12) the significance level of the TTV signal using the metric discussed in Section~\ref{subsec:post_analysis} for candidates with 3$+$ transits (13) scores the candidate gets from the Transmission Spectroscopy Metric \citep[TSM;][]{kemp18}, scaled between 1--100 (14) other names the candidates have and their references. \label{tbl:pc}}
\tablewidth{0pt}
\tabletypesize{\tiny}
\tablehead{
\colhead{TIC ID} & \colhead{$R_\star$} & \colhead{$\rho_\star$} & \colhead{$\rho_{\textrm{circ}}$} & \colhead{$\delta$} & \colhead{$R_{\textrm{p}}$} & \colhead{$b$} & \colhead{$P$} & \colhead{$T_c$} & \colhead{$e$} & \colhead{$\omega$} & \colhead{$\sigma_{\textrm{TTV}}$} & \colhead{TSM} & \colhead{Other Name/Reference}\\ 
\colhead{} & \colhead{[R$_\sun$]} & \colhead{[$\rho_\sun$]} & \colhead{[$\rho_\sun$]} & \colhead{[ppt]} & \colhead{[$R_\earth$]} & \colhead{} & \colhead{[day]} & \colhead{[BJD-2457000]} & \colhead{} & \colhead{[$^\circ$]} & \colhead{} & \colhead{} & \colhead{}
}
\decimalcolnumbers
\startdata
394137592 & 120b & 2.292$^{+0.093}_{-0.093}$ & 0.083$^{+0.007}_{-0.007}$ & 0.114$^{+0.009}_{-0.022}$ & 2.025$^{+0.076}_{-0.057}$ & 11.274$^{+0.497}_{-0.497}$ & 0.234$^{+0.200}_{-0.160}$ & 11.537$^{+0.001}_{-0.001}$ & 1320.543$^{+0.002}_{-0.002}$ & 0.11$^{+0.19}_{-0.11}$ & [-29,40], [133,210] & 0.22$^{+0.027}_{-0.026}$ & 35$^{+9}_{-10}$ & 2.1 & 43 & HD1397b; \citetalias{brah19,niel19} \\
29857954 & 172b & 1.666$^{+0.066}_{-0.066}$ & 0.222$^{+0.032}_{-0.032}$ & 0.574$^{+0.096}_{-0.190}$ & 4.220$^{+0.251}_{-0.242}$ & 11.798$^{+0.596}_{-0.573}$ & 0.307$^{+0.257}_{-0.213}$ & 9.476$^{+0.001}_{-0.001}$ & 1317.444$^{+0.002}_{-0.002}$ & 0.35$^{+0.19}_{-0.23}$ & [-12,66], [113,189] & 0.38$^{+0.0093}_{-0.009}$ & 57$^{+2}_{-2}$ & 0.5 & 12 & \citetalias{rodr19} \\
166739520 & 190b & 1.219$^{+0.043}_{-0.043}$ & 0.563$^{+0.087}_{-0.087}$ & 0.301$^{+0.066}_{-0.068}$ & 7.677$^{+0.362}_{-0.339}$ & 11.656$^{+0.481}_{-0.472}$ & 0.410$^{+0.148}_{-0.241}$ & 10.021$^{+0.000}_{-0.000}$ & 1347.549$^{+0.001}_{-0.001}$ & 0.25$^{+0.26}_{-0.12}$ & [-68,-26], [205,250] & 0.3$^{+0.023}_{-0.023}$ & 242$^{+3}_{-2}$ & 0.9 & 38 & WASP-117b; \citetalias{lend14} \\
183532609 & 191b & 0.957$^{+0.047}_{-0.047}$ & 1.046$^{+0.129}_{-0.129}$ & 0.466$^{+0.085}_{-0.055}$ & 13.215$^{+0.596}_{-0.709}$ & 11.973$^{+0.653}_{-0.651}$ & 0.606$^{+0.052}_{-0.083}$ & 8.159$^{+0.000}_{-0.000}$ & 1350.762$^{+0.000}_{-0.000}$ & 0.29$^{+0.26}_{-0.13}$ & [-71,-27], [209,250] & 0.31$^{+0.0029}_{-0.0024}$ & 274$^{+0}_{-0}$ & 0.5 & 81 & WASP-8b; \citetalias{quel10} \\
410214986 & 200b & 0.913$^{+0.055}_{-0.055}$ & 1.197$^{+1.541}_{-1.541}$ & 1.576$^{+0.163}_{-0.342}$ & 3.591$^{+0.723}_{-0.658}$ & 5.959$^{+0.679}_{-0.659}$ & 0.261$^{+0.209}_{-0.183}$ & 7.872$^{+0.001}_{-0.001}$ & 1332.576$^{+0.001}_{-0.001}$ & 0.11$^{+0.21}_{-0.1}$ & [-32,35], [136,215] & - & - & - & 64 & DS Tuc Ab; \citetalias{newt19} \\
350618622 & 201.01 & 1.229$^{+0.043}_{-0.043}$ & 0.573$^{+0.107}_{-0.107}$ & 3.078$^{+0.833}_{-1.056}$ & 5.390$^{+0.429}_{-0.279}$ & 9.879$^{+0.490}_{-0.445}$ & 0.419$^{+0.204}_{-0.263}$ & 52.978$^{+0.000}_{-0.000}$ & 1323.075$^{+0.001}_{-0.001}$ & 0.55$^{+0.17}_{-0.14}$ & [30,159] & - & - & 1.1 & 29 & \citetalias{hobs21} \\
55652896 & 216b & 0.759$^{+0.044}_{-0.044}$ & 1.793$^{+0.220}_{-0.220}$ & 1.178$^{+0.562}_{-0.279}$ & 9.990$^{+24.072}_{-4.694}$ & 8.311$^{+6.917}_{-2.275}$ & 0.987$^{+0.109}_{-0.055}$ & 17.072$^{+0.001}_{-0.001}$ & 1308.338$^{+0.017}_{-0.017}$ & 0.11$^{+0.28}_{-0.1}$ & [-65,-1], [179,246] & 0.16$^{+0.003}_{-0.002}$ & 292$^{+1}_{-1}$ & 27.1 & 15 & \citetalias{daws21, daws19, kipp19} \\
55652896 & 216c & 0.759$^{+0.044}_{-0.044}$ & 1.793$^{+0.220}_{-0.220}$ & 1.714$^{+0.057}_{-0.096}$ & 15.261$^{+0.281}_{-0.249}$ & 10.232$^{+0.590}_{-0.608}$ & 0.136$^{+0.108}_{-0.092}$ & 34.554$^{+0.001}_{-0.001}$ & 1296.714$^{+0.006}_{-0.006}$ & 0.052$^{+0.21}_{-0.052}$ & [-43,9], [171,222] & 0.0046$^{+0.0027}_{-0.0012}$ & 190$^{+30}_{-50}$ & 24.5 & 15 & \citetalias{daws21, daws19, kipp19} \\
200723869 & 257b & 1.719$^{+0.048}_{-0.048}$ & 0.248$^{+0.035}_{-0.035}$ & 0.380$^{+0.093}_{-0.158}$ & 1.284$^{+0.086}_{-0.061}$ & 6.736$^{+0.289}_{-0.258}$ & 0.389$^{+0.251}_{-0.264}$ & 18.387$^{+0.001}_{-0.001}$ & 1367.377$^{+0.003}_{-0.003}$ & 0.18$^{+0.2}_{-0.16}$ & [-41,49], [137,219] & 0.24$^{+0.04}_{-0.065}$ & 96$^{+22}_{-22}$ & 0.8 & 30 & HD19916b; \citetalias{addi20} \\
339672028 & 481b & 1.605$^{+0.066}_{-0.066}$ & 0.243$^{+0.033}_{-0.033}$ & 0.350$^{+0.056}_{-0.091}$ & 3.878$^{+0.161}_{-0.088}$ & 10.931$^{+0.481}_{-0.468}$ & 0.330$^{+0.199}_{-0.220}$ & 10.331$^{+0.000}_{-0.000}$ & 1377.336$^{+0.001}_{-0.001}$ & 0.11$^{+0.22}_{-0.11}$ & [-30,48], [138,210] & 0.15$^{+0.006}_{-0.007}$ & 65$^{+2}_{-2}$ & 3.3 & 24 & \citetalias{brah20} \\
130415266 & 588.01 & 1.694$^{+0.016}_{-0.016}$ & 0.348$^{+0.009}_{-0.009}$ & 1.018$^{+0.080}_{-0.117}$ & 7.179$^{+0.146}_{-0.101}$ & 15.673$^{+0.202}_{-0.188}$ & 0.250$^{+0.126}_{-0.159}$ & 39.471$^{+0.000}_{-0.000}$ & 1481.793$^{+0.000}_{-0.000}$ & 0.36$^{+0.14}_{-0.071}$ & [27,146] & - & - & - & 87 & - \\
53189332 & 660b & 1.293$^{+0.050}_{-0.050}$ & 0.494$^{+0.077}_{-0.077}$ & 0.393$^{+0.050}_{-0.094}$ & 5.480$^{+0.219}_{-0.220}$ & 10.437$^{+0.458}_{-0.447}$ & 0.277$^{+0.216}_{-0.189}$ & 9.293$^{+0.001}_{-0.001}$ & 1535.348$^{+0.001}_{-0.001}$ & 0.11$^{+0.27}_{-0.098}$ & [-59,-8], [187,240] & - & - & 0.4 & 15 & WASP-106b; \citetalias{smit14} \\
280206394 & 677b & 1.193$^{+0.051}_{-0.051}$ & 0.602$^{+0.093}_{-0.093}$ & 2.241$^{+2.156}_{-0.708}$ & 7.810$^{+0.444}_{-0.833}$ & 11.416$^{+0.651}_{-0.696}$ & 0.705$^{+0.084}_{-0.280}$ & 11.237$^{+0.000}_{-0.000}$ & 1536.233$^{+0.001}_{-0.001}$ & 0.6$^{+0.12}_{-0.25}$ & [26,162] & 0.43$^{+0.024}_{-0.024}$ & 70$^{+4}_{-4}$ & 0.9 & 46 & \citetalias{jord20} \\
286864983 & 772.01 & 0.766$^{+0.042}_{-0.042}$ & 1.746$^{+0.187}_{-0.187}$ & 1.634$^{+0.371}_{-0.628}$ & 5.957$^{+0.398}_{-0.355}$ & 6.443$^{+0.411}_{-0.396}$ & 0.367$^{+0.258}_{-0.249}$ & 11.022$^{+0.003}_{-0.003}$ & 1575.939$^{+0.002}_{-0.002}$ & 0.066$^{+0.28}_{-0.066}$ & [-61,11], [167,238] & - & - & - & 17 & - \\
334305570 & 777.01 & 1.474$^{+0.056}_{-0.056}$ & 0.341$^{+0.062}_{-0.062}$ & 0.871$^{+0.239}_{-0.397}$ & 2.144$^{+0.141}_{-0.116}$ & 7.454$^{+0.367}_{-0.346}$ & 0.400$^{+0.269}_{-0.269}$ & 16.603$^{+0.003}_{-0.003}$ & 1575.780$^{+0.002}_{-0.002}$ & 0.34$^{+0.16}_{-0.28}$ & [-18,51], [104,201] & - & - & - & 13 & - \\
306472057 & 791.01 & 1.279$^{+0.048}_{-0.048}$ & 0.505$^{+0.102}_{-0.102}$ & 0.445$^{+0.097}_{-0.148}$ & 4.461$^{+0.227}_{-0.202}$ & 9.324$^{+0.417}_{-0.411}$ & 0.388$^{+0.215}_{-0.265}$ & 139.309$^{+0.003}_{-0.003}$ & 1427.624$^{+0.002}_{-0.002}$ & 0.077$^{+0.27}_{-0.077}$ & [-60,2], [176,240] & - & - & - & 4 & - \\
363914762 & 812.01 & 1.438$^{+0.048}_{-0.048}$ & 0.403$^{+0.056}_{-0.056}$ & 0.372$^{+0.016}_{-0.039}$ & 6.683$^{+0.112}_{-0.109}$ & 12.816$^{+0.444}_{-0.445}$ & 0.165$^{+0.150}_{-0.113}$ & 13.866$^{+0.000}_{-0.000}$ & 1431.463$^{+0.001}_{-0.001}$ & 0.067$^{+0.23}_{-0.067}$ & [-52,4], [178,228] & - & - & 1.9 & 15 & - \\
158978373 & 823.01 & 1.194$^{+0.045}_{-0.045}$ & 0.606$^{+0.091}_{-0.091}$ & 1.120$^{+0.666}_{-0.787}$ & 1.993$^{+0.506}_{-0.246}$ & 5.837$^{+0.711}_{-0.451}$ & 0.529$^{+0.306}_{-0.357}$ & 13.540$^{+0.005}_{-0.005}$ & 1609.005$^{+0.003}_{-0.003}$ & 0.32$^{+0.19}_{-0.27}$ & [-45,58], [124,220] & - & - & - & 10 & - \\
243200602 & 826.01 & 0.975$^{+0.045}_{-0.045}$ & 0.983$^{+0.118}_{-0.118}$ & 1.347$^{+0.412}_{-0.497}$ & 8.556$^{+0.665}_{-0.533}$ & 9.866$^{+0.551}_{-0.536}$ & 0.447$^{+0.212}_{-0.286}$ & 11.554$^{+0.001}_{-0.001}$ & 1607.581$^{+0.001}_{-0.001}$ & 0.12$^{+0.24}_{-0.11}$ & [-42,41], [141,220] & - & - & - & 26 & WASP-130b; \citetalias{hell17} \\
123846039 & 883.01 & 0.967$^{+0.043}_{-0.043}$ & 1.011$^{+0.117}_{-0.117}$ & 0.944$^{+0.401}_{-0.545}$ & 3.863$^{+0.483}_{-0.276}$ & 6.583$^{+0.453}_{-0.387}$ & 0.486$^{+0.279}_{-0.326}$ & 10.051$^{+0.002}_{-0.002}$ & 1476.531$^{+0.001}_{-0.001}$ & 0.091$^{+0.31}_{-0.086}$ & [-63,17], [161,245] & - & - & - & 28 & - \\
177162886 & 899.01 & 1.051$^{+0.049}_{-0.049}$ & 0.834$^{+1.541}_{-1.541}$ & 2.265$^{+1.237}_{-0.961}$ & 7.264$^{+0.935}_{-0.615}$ & 9.823$^{+0.695}_{-0.624}$ & 0.563$^{+0.194}_{-0.303}$ & 12.846$^{+0.000}_{-0.000}$ & 1313.638$^{+0.001}_{-0.001}$ & 0.45$^{+0.18}_{-0.2}$ & [10,65], [89,174] & - & - & 2.7 & 12 & - \\
260130483 & 933.01 & 1.644$^{+0.070}_{-0.070}$ & 0.210$^{+0.038}_{-0.038}$ & 0.313$^{+0.173}_{-0.067}$ & 4.210$^{+0.220}_{-0.237}$ & 11.603$^{+0.596}_{-0.652}$ & 0.817$^{+0.033}_{-0.089}$ & 88.932$^{+0.001}_{-0.001}$ & 1256.009$^{+0.002}_{-0.002}$ & 0.13$^{+0.36}_{-0.1}$ & [-22,67], [133,198] & - & - & 0.3 & 4 & - \\
408137826 & 941.01 & 1.070$^{+0.047}_{-0.047}$ & 0.755$^{+0.107}_{-0.107}$ & 0.698$^{+0.276}_{-0.394}$ & 2.997$^{+0.340}_{-0.271}$ & 6.393$^{+0.455}_{-0.412}$ & 0.441$^{+0.299}_{-0.303}$ & 8.511$^{+0.001}_{-0.001}$ & 1431.971$^{+0.001}_{-0.001}$ & 0.084$^{+0.32}_{-0.082}$ & [-65,12], [162,245] & - & - & 0.2 & 10 & - \\
399871011 & 943.01 & 1.284$^{+0.050}_{-0.050}$ & 0.496$^{+0.099}_{-0.099}$ & 0.362$^{+0.078}_{-0.144}$ & 6.490$^{+0.365}_{-0.351}$ & 11.283$^{+0.551}_{-0.533}$ & 0.375$^{+0.264}_{-0.260}$ & 12.360$^{+0.002}_{-0.002}$ & 1444.268$^{+0.002}_{-0.002}$ & 0.12$^{+0.31}_{-0.1}$ & [-66,-10], [193,244] & - & - & - & 16 & - \\
25799609 & 963.01 & 1.015$^{+0.041}_{-0.041}$ & 0.879$^{+0.113}_{-0.113}$ & 0.341$^{+0.617}_{-0.131}$ & 5.802$^{+0.403}_{-0.528}$ & 8.409$^{+0.466}_{-0.494}$ & 0.761$^{+0.073}_{-0.392}$ & 11.114$^{+0.003}_{-0.003}$ & 1501.309$^{+0.002}_{-0.002}$ & 0.094$^{+0.38}_{-0.075}$ & [-77,3], [179,255] & - & - & - & 18 & - \\
73038411 & 978.01 & 1.434$^{+0.054}_{-0.054}$ & 0.392$^{+0.060}_{-0.060}$ & 0.847$^{+0.180}_{-0.232}$ & 5.801$^{+0.833}_{-0.785}$ & 11.910$^{+0.937}_{-0.945}$ & 0.289$^{+0.227}_{-0.200}$ & 15.854$^{+1.437}_{-1.437}$ & 1502.778$^{+0.002}_{-0.002}$ & 0.3$^{+0.21}_{-0.21}$ & [-13,62], [113,195] & - & - & - & 17 & - \\
254113311 & 1130c & 0.695$^{+0.036}_{-0.036}$ & 2.195$^{+0.265}_{-0.265}$ & 1.920$^{+0.478}_{-0.250}$ & 35.686$^{+76.608}_{-16.610}$ & 14.292$^{+11.245}_{-3.810}$ & 0.986$^{+0.182}_{-0.091}$ & 8.351$^{+0.000}_{-0.000}$ & 1649.547$^{+0.001}_{-0.001}$ & 0.073$^{+0.22}_{-0.073}$ & [-51,12], [168,230] & 0.047$^{+0.04}_{-0.027}$ & 332$^{+24}_{-55}$ & 1.1 & 100 & \citetalias{huan20} \\
409794137 & 1478b & 0.988$^{+0.044}_{-0.044}$ & 0.974$^{+0.126}_{-0.126}$ & 1.116$^{+0.200}_{-0.333}$ & 8.944$^{+0.502}_{-0.358}$ & 10.213$^{+0.525}_{-0.509}$ & 0.339$^{+0.218}_{-0.225}$ & 10.181$^{+0.000}_{-0.000}$ & 1485.738$^{+0.001}_{-0.001}$ & 0.085$^{+0.23}_{-0.085}$ & [-44,30], [153,224] & 0.024$^{+0.032}_{-0.017}$ & 250$^{+120}_{-130}$ & 1.0 & 33 & \citetalias{rodr21} \\
308098254 & 1906.01 & 1.113$^{+0.048}_{-0.048}$ & 0.701$^{+0.090}_{-0.090}$ & 0.619$^{+0.260}_{-0.269}$ & 8.517$^{+0.903}_{-0.613}$ & 11.249$^{+0.710}_{-0.648}$ & 0.494$^{+0.214}_{-0.318}$ & 9.627$^{+0.000}_{-0.000}$ & 1538.718$^{+0.000}_{-0.000}$ & 0.087$^{+0.28}_{-0.083}$ & [-62,12], [168,241] & 0.43$^{+0.005}_{-0.005}$ & 358$^{+2}_{-2}$ & 0.1 & 15 & WASP-162b; \citetalias{hell19} \\
190271688 & 1963.01 & 1.062$^{+0.054}_{-0.054}$ & 0.776$^{+0.107}_{-0.107}$ & 0.814$^{+0.097}_{-0.073}$ & 21.059$^{+0.777}_{-1.058}$ & 16.751$^{+0.922}_{-0.912}$ & 0.659$^{+0.036}_{-0.051}$ & 12.636$^{+0.001}_{-0.001}$ & 1607.245$^{+0.000}_{-0.000}$ & 0.055$^{+0.22}_{-0.055}$ & [-35,26], [152,213] & - & - & - & 57 & - \\
371188886 & 2000.01 & 1.074$^{+0.053}_{-0.053}$ & 0.769$^{+0.104}_{-0.104}$ & 1.221$^{+0.298}_{-0.544}$ & 3.730$^{+0.258}_{-0.200}$ & 7.160$^{+0.433}_{-0.405}$ & 0.389$^{+0.273}_{-0.261}$ & 9.127$^{+0.001}_{-0.001}$ & 1535.058$^{+0.003}_{-0.003}$ & 0.19$^{+0.2}_{-0.17}$ & [-41,51], [137,221] & - & - & 2.3 & 16 & - \\
147660886 & 2005.01 & 2.103$^{+0.077}_{-0.077}$ & 0.161$^{+0.021}_{-0.021}$ & 1.394$^{+0.314}_{-0.559}$ & 2.498$^{+0.164}_{-0.149}$ & 11.461$^{+0.578}_{-0.546}$ & 0.366$^{+0.257}_{-0.250}$ & 17.306$^{+0.002}_{-0.002}$ & 1549.835$^{+0.002}_{-0.002}$ & 0.65$^{+0.14}_{-0.15}$ & [29,148] & - & - & - & 13 & - \\
394287035 & 2328.01 & 0.829$^{+0.042}_{-0.042}$ & 1.429$^{+0.167}_{-0.167}$ & 2.693$^{+0.508}_{-0.937}$ & 9.130$^{+0.598}_{-0.538}$ & 8.639$^{+0.519}_{-0.504}$ & 0.327$^{+0.254}_{-0.219}$ & 17.102$^{+0.000}_{-0.000}$ & 1313.386$^{+0.000}_{-0.000}$ & 0.24$^{+0.18}_{-0.22}$ & [-27,52], [123,209] & - & - & 0.1 & 14 & CTOI \\
24358417 & 2338.01 & 1.028$^{+0.047}_{-0.047}$ & 0.881$^{+0.125}_{-0.125}$ & 3.631$^{+0.592}_{-1.020}$ & 10.028$^{+0.508}_{-0.547}$ & 11.218$^{+0.600}_{-0.595}$ & 0.278$^{+0.230}_{-0.191}$ & 22.652$^{+0.003}_{-0.003}$ & 1481.407$^{+0.002}_{-0.002}$ & 0.48$^{+0.2}_{-0.15}$ & [20,55], [68,170] & - & - & - & 11 & - \\
279514271 & 2339.01 & 2.166$^{+0.096}_{-0.096}$ & 0.086$^{+0.015}_{-0.015}$ & 0.085$^{+0.050}_{-0.059}$ & 2.032$^{+0.526}_{-0.239}$ & 10.720$^{+1.334}_{-0.862}$ & 0.528$^{+0.297}_{-0.355}$ & 9.774$^{+0.000}_{-0.000}$ & 1351.802$^{+0.008}_{-0.008}$ & 0.13$^{+0.29}_{-0.11}$ & [-64,29], [152,243] & - & - & 1.2 & 1 & - \\
204671232 & 2361.01 & 0.984$^{+0.045}_{-0.045}$ & 0.971$^{+0.125}_{-0.125}$ & 1.001$^{+0.134}_{-0.230}$ & 10.749$^{+0.520}_{-0.539}$ & 11.114$^{+0.572}_{-0.565}$ & 0.259$^{+0.212}_{-0.177}$ & 8.716$^{+0.003}_{-0.003}$ & 1569.062$^{+0.007}_{-0.007}$ & 0.062$^{+0.24}_{-0.062}$ & [-47,19], [160,228] & - & - & 2.3 & 15 & CTOI; \citetalias{mont20} \\
238542895 & - & 0.896$^{+0.030}_{-0.030}$ & 1.204$^{+0.137}_{-0.137}$ & 0.730$^{+0.076}_{-0.136}$ & 10.233$^{+0.431}_{-0.432}$ & 9.872$^{+0.398}_{-0.391}$ & 0.229$^{+0.203}_{-0.157}$ & 8.385$^{+0.000}_{-0.000}$ & 1485.880$^{+0.001}_{-0.001}$ & 0.21$^{+0.27}_{-0.094}$ & [-66,-24], [203,247] & - & - & 1.6 & 18 & CTOI \\
282498590 & - & 1.051$^{+0.145}_{-0.145}$ & 0.778$^{+0.279}_{-0.279}$ & 0.556$^{+0.101}_{-0.172}$ & 10.780$^{+0.656}_{-0.543}$ & 11.896$^{+1.674}_{-1.603}$ & 0.343$^{+0.231}_{-0.232}$ & 10.095$^{+0.002}_{-0.002}$ & 1474.825$^{+0.001}_{-0.001}$ & 0.16$^{+0.27}_{-0.14}$ & [-66,-8], [189,246] & - & - & - & 22 & CTOI; \citetalias{mont20}  \\
290403522 & - & 1.384$^{+0.052}_{-0.052}$ & 0.435$^{+0.067}_{-0.067}$ & 0.059$^{+0.010}_{-0.007}$ & 6.596$^{+0.231}_{-0.246}$ & 12.247$^{+0.512}_{-0.499}$ & 0.538$^{+0.057}_{-0.092}$ & 22.375$^{+0.000}_{-0.000}$ & 1324.188$^{+0.003}_{-0.003}$ & 0.61$^{+0.16}_{-0.076}$ & [-86,-52], [232,266] & - & - & 1.5 & 18 & CTOI \\
380836882 & - & 1.197$^{+0.053}_{-0.053}$ & 0.574$^{+0.087}_{-0.087}$ & 0.392$^{+0.052}_{-0.102}$ & 6.541$^{+0.367}_{-0.302}$ & 10.573$^{+0.553}_{-0.534}$ & 0.282$^{+0.219}_{-0.195}$ & 8.012$^{+0.000}_{-0.000}$ & 1652.826$^{+0.001}_{-0.001}$ & 0.17$^{+0.28}_{-0.11}$ & [-65,-17], [197,243] & - & - & 0.3 & 18 & CTOI \\
382200986 & - & 0.680$^{+0.036}_{-0.036}$ & 2.182$^{+0.232}_{-0.232}$ & 2.002$^{+0.251}_{-0.449}$ & 8.810$^{+0.417}_{-0.346}$ & 6.975$^{+0.399}_{-0.394}$ & 0.279$^{+0.202}_{-0.191}$ & 92.498$^{+0.005}_{-0.005}$ & 1243.912$^{+0.010}_{-0.010}$ & 0.06$^{+0.25}_{-0.06}$ & [-51,1], [175,233] & - & - & 3.7 & 5 & CTOI; \citetalias{mont20} \\
357202877 & - & 1.116$^{+0.044}_{-0.044}$ & 0.645$^{+0.084}_{-0.084}$ & 1.143$^{+0.693}_{-0.549}$ & 14.388$^{+3.440}_{-2.518}$ & 14.643$^{+1.728}_{-1.468}$ & 0.570$^{+0.223}_{-0.372}$ & 9.555$^{+0.001}_{-0.001}$ & 1534.787$^{+0.003}_{-0.003}$ & 0.1$^{+0.33}_{-0.084}$ & [-35,56], [132,213] & - & - & 1.0 & 20 & - \\
254142310 & - & 1.633$^{+0.074}_{-0.074}$ & 0.231$^{+0.045}_{-0.045}$ & 0.264$^{+0.080}_{-0.123}$ & 2.986$^{+0.322}_{-0.252}$ & 9.743$^{+0.675}_{-0.616}$ & 0.414$^{+0.267}_{-0.279}$ & 9.311$^{+0.002}_{-0.002}$ & 1652.052$^{+0.004}_{-0.004}$ & 0.11$^{+0.27}_{-0.099}$ & [-57,27], [152,236] & - & - & 0.6 & 8 & - \\
395113305 & - & 0.886$^{+0.043}_{-0.043}$ & 1.272$^{+0.162}_{-0.162}$ & 0.284$^{+0.150}_{-0.159}$ & 7.345$^{+1.252}_{-0.917}$ & 8.294$^{+0.787}_{-0.667}$ & 0.506$^{+0.259}_{-0.338}$ & 9.963$^{+0.008}_{-0.008}$ & 1607.420$^{+0.006}_{-0.006}$ & 0.48$^{+0.27}_{-0.1}$ & [-82,-45], [224,262] & - & - & - & 11 & - \\
180989820 & - & 1.256$^{+0.058}_{-0.058}$ & 0.544$^{+0.088}_{-0.088}$ & 0.084$^{+0.017}_{-0.026}$ & 4.508$^{+0.338}_{-0.236}$ & 9.223$^{+0.524}_{-0.484}$ & 0.356$^{+0.216}_{-0.243}$ & 9.873$^{+0.001}_{-0.001}$ & 1511.287$^{+0.004}_{-0.004}$ & 0.63$^{+0.14}_{-0.1}$ & [-86,-52], [233,265] & - & - & 1.4 & 12 & - \\
4598935 & - & 1.042$^{+0.040}_{-0.040}$ & 0.801$^{+0.108}_{-0.108}$ & 0.460$^{+0.159}_{-0.231}$ & 3.515$^{+0.475}_{-0.367}$ & 6.744$^{+0.525}_{-0.455}$ & 0.438$^{+0.271}_{-0.299}$ & 24.663$^{+0.007}_{-0.007}$ & 1539.451$^{+0.006}_{-0.006}$ & 0.19$^{+0.35}_{-0.12}$ & [-71,-19], [202,248] & - & - & - & 5 & - \\
464300749 & - & 1.678$^{+0.056}_{-0.056}$ & 0.270$^{+0.044}_{-0.044}$ & 4.896$^{+1.439}_{-2.229}$ & 4.007$^{+0.334}_{-0.316}$ & 11.589$^{+0.620}_{-0.601}$ & 0.385$^{+0.281}_{-0.265}$ & 18.098$^{+0.003}_{-0.003}$ & 1529.321$^{+0.006}_{-0.006}$ & 0.78$^{+0.098}_{-0.13}$ & [34,143] & - & - & 1.1 & 11 & - \\
7536985 & - & 1.908$^{+0.086}_{-0.086}$ & 0.163$^{+0.036}_{-0.036}$ & 0.315$^{+0.091}_{-0.133}$ & 7.271$^{+0.557}_{-0.503}$ & 17.745$^{+1.074}_{-1.015}$ & 0.397$^{+0.253}_{-0.268}$ & 12.732$^{+0.005}_{-0.005}$ & 1502.907$^{+0.004}_{-0.004}$ & 0.25$^{+0.19}_{-0.22}$ & [-32,54], [128,210] & - & - & - & 8 & - \\
76228620 & - & 1.194$^{+0.051}_{-0.051}$ & 0.571$^{+0.090}_{-0.090}$ & 0.343$^{+0.227}_{-0.217}$ & 4.492$^{+1.118}_{-0.626}$ & 8.768$^{+1.045}_{-0.768}$ & 0.567$^{+0.254}_{-0.381}$ & 9.779$^{+0.002}_{-0.002}$ & 1645.400$^{+0.004}_{-0.004}$ & 0.078$^{+0.37}_{-0.075}$ & [-71,-4], [186,253] & - & - & 0.5 & 11 & - \\
87422071 & - & 1.342$^{+0.055}_{-0.055}$ & 0.413$^{+0.073}_{-0.073}$ & 0.794$^{+0.358}_{-0.447}$ & 3.622$^{+0.524}_{-0.433}$ & 8.803$^{+0.753}_{-0.660}$ & 0.444$^{+0.295}_{-0.304}$ & 11.366$^{+0.004}_{-0.004}$ & 1646.564$^{+0.008}_{-0.008}$ & 0.29$^{+0.19}_{-0.24}$ & [-35,58], [121,216] & - & - & 0.7 & 8 & - \\
253126207 & - & 1.249$^{+0.046}_{-0.046}$ & 0.506$^{+0.085}_{-0.085}$ & 1.547$^{+0.208}_{-0.325}$ & 11.792$^{+0.551}_{-0.588}$ & 14.784$^{+0.648}_{-0.646}$ & 0.255$^{+0.207}_{-0.174}$ & 17.434$^{+0.002}_{-0.002}$ & 1604.089$^{+0.001}_{-0.001}$ & 0.39$^{+0.22}_{-0.12}$ & [8,77], [101,172] & - & - & - & 22 & - \\
342167886 & - & 1.437$^{+0.095}_{-0.095}$ & 0.348$^{+0.080}_{-0.080}$ & 0.983$^{+0.153}_{-0.318}$ & 7.701$^{+0.314}_{-0.353}$ & 13.731$^{+0.963}_{-0.967}$ & 0.313$^{+0.248}_{-0.218}$ & 17.308$^{+0.001}_{-0.001}$ & 1510.187$^{+0.003}_{-0.003}$ & 0.36$^{+0.22}_{-0.19}$ & [-4,60], [105,188] & - & - & 1.5 & 11 & - \\
343936388 & - & 0.855$^{+0.033}_{-0.033}$ & 1.350$^{+0.155}_{-0.155}$ & 0.303$^{+0.228}_{-0.184}$ & 4.702$^{+0.584}_{-0.489}$ & 6.397$^{+0.454}_{-0.409}$ & 0.583$^{+0.227}_{-0.389}$ & 15.144$^{+0.009}_{-0.009}$ & 1469.040$^{+0.019}_{-0.019}$ & 0.48$^{+0.26}_{-0.15}$ & [-81,-42], [222,261] & - & - & 1.9 & 6 & - \\
394492336 & - & 0.934$^{+0.044}_{-0.044}$ & 1.063$^{+0.113}_{-0.113}$ & 3.489$^{+1.140}_{-1.470}$ & 11.543$^{+1.345}_{-0.961}$ & 10.975$^{+0.776}_{-0.699}$ & 0.436$^{+0.243}_{-0.286}$ & 9.131$^{+0.000}_{-0.000}$ & 1597.926$^{+0.002}_{-0.002}$ & 0.43$^{+0.19}_{-0.24}$ & [4,63], [95,183] & - & - & 1.4 & 22 & - \\
150299840 & - & 1.839$^{+0.061}_{-0.061}$ & 0.220$^{+0.031}_{-0.031}$ & 0.443$^{+0.046}_{-0.096}$ & 5.362$^{+0.422}_{-0.369}$ & 14.685$^{+0.740}_{-0.699}$ & 0.259$^{+0.202}_{-0.175}$ & 19.473$^{+0.001}_{-0.001}$ & 1308.841$^{+0.005}_{-0.005}$ & 0.27$^{+0.24}_{-0.14}$ & [-6,65], [116,190] & - & - & 3.7 & 13 & - \\
\enddata
\tablecomments{Stellar parameters $R_\star$ and $\rho_\star$ are derived from the isochrone fitting (Section~\ref{sec:selection}). Planet parameters $\rho_{\textrm{circ}}$, $\delta$, $R_{\textrm{p}}$, $b$, $P$, $T_c$, $e$, and $\omega$ are derived from the light curve fitting (Section~\ref{sec:lc}). We report the medians and 68\% credible intervals of posteriors for all parameters except for $e$ and $\omega$. For $e$, we report the modes and 68\% highest posterior density (HPD) intervals. For $\omega$, we report the 68\% HPD intervals of which have taken account of multimodal distributions.}
\tablerefs{Reference abbreviations used in this able are listed. Br19: \cite{brah19}; Ni9: \cite{niel19}; Ro19: \cite{rodr19}; Le14: \cite{lend14}; Qu10: \cite{quel10}; Ne19: \cite{newt19}; Ho21: \cite{hobs21}; Da21: \cite{daws21}; Da19: \cite{daws19}; Ki19: \cite{kipp19}; Ad20: \cite{addi20}; Br20: \cite{brah20}; Sm14: \cite{smit14}; Jo20: \cite{jord20}; He17: \cite{hell17}; Hu20: \cite{huan20}; He19: \cite{hell19}.}
\end{deluxetable*}
\end{longrotatetable}

==> Tables/PC_grazing.tex <==
\begin{deluxetable*}{lcc}
\tablecaption{Possible WaLEs candidates with unconstrained radii. \label{tbl:pc_grazing}}
\tabletypesize{\small}
\tablehead{
\colhead{TIC ID} & \colhead{TOI name} & \colhead{Comment/Reference}
}
\startdata
384164973 & - & - \\
38815574 & - & -\\
4588737 & - & -\\
117817010 & - & -\\
359271114 & - & -\\
379717270 & - & -\\
381982417 & - & -\\
410395660 & - & -\\
412484721 & - & -\\
460205581 & TOI-837.01 & \cite{boum20} \\
461968320 & - & -\\
464124454 & - & -\\
467807116 & - & -\\
76761591 & - & -\\
304418238 & - & -\\
305345992 & - & -\\
359732062 & - & -\\
462162948 & TOI-684.01 & -\\
467807015 & - & -\\
\enddata
\tablecomments{These candidates are not included in our catalog.}
\end{deluxetable*}
